Edge-Enhanced Vision Transformer Framework for Accurate AI-Generated Image Detection

The rapid advancement of generative models has led to a growing prevalence of highly realistic AI-generated images, posing significant challenges for digital forensics and content authentication. Conventional detection methods mainly rely on deep learning models that extract global features, which often overlook subtle structural inconsistencies and demand substantial computational resources. To address these limitations, we propose a hybrid detection framework that combines a fine-tuned Vision Transformer (ViT) with a novel edge-based image processing module. The edge-based module computes variance from edge-difference maps generated before and after smoothing, exploiting the observation that AI-generated images typically exhibit smoother textures, weaker edges, and reduced noise compared to real images. When applied as a post-processing step on ViT predictions, this module enhances sensitivity to fine-grained structural cues while maintaining computational efficiency. Extensive experiments on the CIFAKE, Artistic, and Custom Curated datasets demonstrate that the proposed framework achieves superior detection performance across all benchmarks, attaining 97.75% accuracy and a 97.77% F1-score on CIFAKE, surpassing widely adopted state-of-the-art models. These results establish the proposed method as a lightweight, interpretable, and effective solution for both still images and video frames, making it highly suitable for real-world applications in automated content verification and digital forensics.

==> temp.tex <==
\section{Related Work}
\label{related work}

In recent years, research on detecting AI-generated images has grown rapidly. This is largely driven by the progress of generative models and the highly realistic images they can produce. In this section, we summarize the major approaches and findings from prior work.

\subsection{Benchmarks and Datasets}
The representativeness and diversity of detection benchmarks have become central concerns in evaluating AI-image detectors. Curated datasets such as GenImage~\cite{boychev2024bench}, Chameleon~\cite{yan2024sanity}, and ITW-SM~\cite{konstantinidou2025navigating} attempt to capture realistic distributions by aggregating images from social platforms, varied generators (GANs, diffusion, transformers), and multiple domains. GenImage compiles millions of samples from open-source models as well as proprietary tools like Midjourney and Stable Diffusion, allowing cross-model performance comparisons. However, even the largest datasets fall short in capturing the pace of generative progress, with new architectures quickly rendering existing benchmarks obsolete. ITW-SM uniquely focuses on distribution shift and adversarial perturbations, including images undergoing social platform compression and style transfer; here, SOTA models frequently exhibit up to 40\% accuracy reduction compared to canonical benchmarks, exposing their fragility. Further, annotation inaccuracies and domain mismatches manifest as annotation bias in these datasets~\cite{jiang2023domainadapt}, complicating reproducible cross-paper comparisons. Emerging efforts combine active curation and continual benchmarking, but automated annotation pipelines remain a critical bottleneck.

\subsection{CNN and Hybrid Models}
Convolutional neural network (CNN) based discriminators have provided the backbone for early AI-image detection, especially those trained to distinguish low-level statistical artifacts in GAN output. DMID~\cite{konstantinidou2025navigating} and multi-view fusion networks~\cite{liu2023analysis} integrate color, texture, and deep features, with multi-branch ensembles boosting robustness to generator variation. Yet, these architectures often operate as black-box classifiers, inheriting vulnerabilities to distribution shifts: images generated by novel GAN or diffusion models regularly evade detection~\cite{gragnaniello2021generalization}. Patch-based CNN methods~\cite{chen2024patchdet} and hybrid spectral-CNN ensembles~\cite{karageorgiou2025spectral} extend detection beyond single-source images by analyzing frequency domain and spatial patches, further integrating compressed and manipulated inputs. However, these approaches typically sacrifice processing speed and scalability, relying on computationally expensive grid or Fourier transforms. Few-shot learning methods, notably FSD~\cite{wu2024fewshot}, enable detectors to generalize from minimal annotated samples, accelerating adaptation to new architectures. Still, limitations persist: when confronted with highly quantized or proprietary models (e.g., VQDM), few-shot detectors fail to capture core distributional nuances due to insufficient representation learning.

\subsection{Transformer and Vision-Language Architectures}
Transformer-based models revolutionized synthetic image detection by embedding both global context and semantic associations. CLIP~\cite{radford2021learning} and DINO-V2~\cite{oquab2023dinov2} pioneered large-scale pretraining, enabling robust recognition of subtle generative cues from text-image pairs. BLIP2~\cite{li2023blip}, ZeroVIL~\cite{liu2024zerovil}, and FAKEINVERSION~\cite{cazenavette2024fakeinversion} augment feature space with vision-language alignment, substantially improving domain transfer and zero-shot capabilities. State-of-the-art transformer detectors leverage attention maps to localize artifacts such as anomalous texture blending, boundary artifacts, and atypical semantic correlations. Cross-modal architectures—using both spatial and textual attributes—further mitigate overfitting to specific generators, as seen in BLIP2 and ZeroVIL performance on unseen models~\cite{zhang2024comprehensive}. Despite these advances, the pretraining cost and data requirements for successful transformers remain prohibitively high, often restricting practical deployment. Additionally, adversarial attacks and heavy annotation noise—such as robust JPEG compression or manipulated captions—introduce substantial perturbation to transformer-based discriminators; accuracy downside may range from 95\% to 65\% in real-world benchmarks~\cite{saberi2023robustness}.

\subsection{Cross-Generator and Patch-Based Detection}
To address the diversity of modern generative models, recent strategies center on patch-level and spectral learning. PatchDet~\cite{chen2024patchdet} segments images into overlapping regions, analyzing pattern recurrence and artifact density, especially for diffusion-based and mixed-modality generators. Spectral learning~\cite{karageorgiou2025spectral} employs Fourier and eigen decomposition to identify subtle periodic or frequency domain deviations that escape holistic classifiers. These methods excel in identifying images with localized manipulations or hidden generator traces, showing up to 20\% improvement in mixed-domain detection. Limitations, however, include increased latency (due to region-wise inference) and reduced generalization on images with global postprocessing, such as color remapping or cross-domain transformation. Ensemble patch-spectral architectures blend local and global features, but require careful calibration to avoid redundancy and computational overload; ablation studies show diminishing returns as patch count increases beyond a threshold.

\subsection{Diffusion and Autoencoder Reconstructions}
The surge in diffusion-based generators prompted detector design based on reconstruction error and latent statistics. DIRE~\cite{wang2023dire}, LARE2~\cite{luo2024lare2}, and SeDID~\cite{ma2023sedid} use autoencoder and stepwise latent error modeling to flag unrealistic synthesis patterns. These reconstruction-driven approaches outperform direct feature-based detectors against open-source diffusion and transformer models, especially by exploiting generative smoothing and blending trends in the latent space. However, on closed-source or proprietary algorithms, where reconstruction style diverges from training assumptions, accuracy may decrease by up to 30\%. Further, latent reconstruction methods require heavy computational resources and fine-tuning, reducing the feasibility of real-time inference for large-scale deployments. Integration with transformer backbones provides some robustness, but the need for careful hyperparameter selection and bespoke regularization (e.g., manifold alignment) complicates practical adoption.

\subsection{Watermarking and Robustness Studies}
Robustness-centric studies probe the practical vulnerabilities of current detectors, especially in adversarial and counter-forensic scenarios. Watermarking methods~\cite{saberi2023robustness} embed detectable patterns during synthesis or postprocessing, designed to signal image provenance. However, adaptive attackers can evade detection by applying image purification, enhancement, or re-synthesis via robust diffusion pipelines, nullifying the watermark signal. Classifier-based detectors are also subject to distributional and adversarial attacks, including paraphrasing, cropping, and style transfer; practical studies~\cite{boychev2024bench, zhang2024comprehensive} show classifier error rates can double after active evasion. Efforts to merge watermarking with multi-expert ensembles (spatial, frequency, semantic) have improved resilience but at the cost of model complexity and real-world generalization. Moreover, no single watermark or classifier strategy currently survives persistent, adaptive adversarial manipulation over extended timelines.

\subsection{Edge and Lightweight Deep Learning}
Real-time detection and deployment constraints have fueled research into edge-compatible and lightweight deep learning models. Surveys~\cite{mittal2024edgedeep, zhou2021lightweight, albahri2021lightweight, liu2023edge, zou2023object} summarize compact CNN and transformer alternatives for mobile and hardware-limited platforms. Compression, pruning, and quantization lower memory and computational footprints, enabling practical, power-efficient detectors. Recent lightweight detectors maintain close-to-SOTA accuracy on well-structured datasets, but trade off fine discrimination: edge-centric or lightweight models sometimes misclassify high-fidelity synthetics or heavily compressed outputs, as demonstrated in medical and multimedia diagnostic tasks. Multi-scale feature selection and adaptive inference pipelines are proposed to mitigate these losses, but deployment remains constrained outside controlled environments due to input dimensionality and reduced robustness.

\subsection{Ensemble and Multi-Expert Methods}
Recent works have shown pronounced benefits from combining multiple models—or modalities—through ensemble learning. Weighted and stacking ensembles~\cite{anan2025hybrid, wolter2023wavelet, gowda2023ensemble, wodajo2022cnn, ricker2024aeroblade} are used to merge CNNs (like SEResNet or XceptionNet), Transformers, and frequency-domain networks. For instance, the DFWild-Cup ensemble leverages ResNet-34, DeiT, and XceptionNet with Haar wavelet features to yield 93\% accuracy and 0.97 ROC-AUC~\cite{kafi2025hybrid}. Stacking architectures~\cite{wolter2023wavelet, waterman2024ensemble} employ meta-learners to combine base model votes for sky-high reliability. A limitation is increased computational overhead and memory usage, often constraining ensemble deployment in real-time and edge settings. Additionally, effective ensemble weights require extensive hyperparameter tuning, and generalization may still be reduced on out-of-domain generator styles unless specifically robustified by adversarial training.

\subsection{Self-Supervised Learning and Feature Engineering}
Self-supervised learning has recently emerged as a powerful tool for cross-generator generalization. BLADES~\cite{zou2025bilevel} introduces bi-level optimization to tailor pretext objectives (e.g., EXIF tag prediction, manipulation detection) to downstream AI-generated image detection, even without synthetic images in pretraining. This method delivers SOTA results on face detection: it combines EXIF-based linguistic embeddings with surrogate tasks like coarse-grained and fine-grained manipulation detection, utilizing task-aware dynamic weighting for maximal discriminative power. Masked autoencoders (MAE), PATCHForensics~\cite{zhou2023masked}, and frequency-based SSL~\cite{wolter2023wavelet} also enhance feature separation. However, self-supervised approaches often rely on indirect cues: if pretext losses are not optimal for detection, performance may lag behind supervised methods, especially on subtle manipulations or novel synthetic domains.
Overall, advances increasingly target hybrid solutions, deploying both local patchwise and global semantic context, with transformers and lightweight networks jointly mitigating weaknesses. These trends motivate our hybrid edge-transformer detection approach, aiming to balance accuracy, generalization, and computational efficiency.
